Solving, Tracking and Stopping Streaming Linear Inverse Problems

In large-scale applications including medical imaging, collocation differential equation solvers, and estimation with differential privacy, the underlying linear inverse problem can be reformulated as a streaming problem. In theory, the streaming problem can be effectively solved using memory-efficient, exponentially-converging streaming solvers. In practice, a streaming solver's effectiveness is undermined if it is stopped before, or well-after, the desired accuracy is achieved. In special cases when the underlying linear inverse problem is finite-dimensional, streaming solvers can periodically evaluate the residual norm at a substantial computational cost. When the underlying system is infinite dimensional, streaming solver can only access noisy estimates of the residual. While such noisy estimates are computationally efficient, they are useful only when their accuracy is known. In this work, we rigorously develop a general family of computationally-practical residual estimators and their uncertainty sets for streaming solvers, and we demonstrate the accuracy of our methods on a number of large-scale linear problems. Thus, we further enable the practical use of streaming solvers for important classes of linear inverse problems.

==> plots/plots/ci_table_noeta.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Apr 26 13:45:46 2022
\begin{longtable}{lrlrrlllll}
  \hline
Sampling Method & Width & Matrix Type & Rows & eta & $>10$ & $>1e-5$ & $>1e-10$ & $>0$ & Total \\ 
  \hline
Achlio & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}2e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}2e-04 \\ 
  Achlio & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}1e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}1e-04 \\ 
  Achlio & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}2e-04 & \cellcolor{white}0 & \cellcolor{white}2e-04 \\ 
  Achlio & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}5e-04 & \cellcolor{white}0 & \cellcolor{white}5e-04 \\ 
  gauss & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}1e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}1e-04 \\ 
  gauss & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}3e-04 & \cellcolor{white}0 & \cellcolor{white}3e-04 \\ 
  gauss & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
   \hline
\hline
\end{longtable}


==> plots/plots/eta_tab.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue May 17 15:17:54 2022
\begin{longtable}{llrrr}
  \hline
Width & Percent Sampled & Achlio & FJLT & gauss \\ 
  \hline
15 & 0.04 & 5 & 82 & 5 \\ 
  15 & 0.1 & 6 & 91 & 6 \\ 
  15 & 0.39 & 9 & 134 & 9 \\ 
  30 & 0.04 & 6 & 101 & 6 \\ 
  30 & 0.1 & 7 & 106 & 7 \\ 
  30 & 0.39 & 10 & 153 & 11 \\ 
  100 & 0.04 & 9 & 129 & 8 \\ 
  100 & 0.1 & 9 & 141 & 9 \\ 
  100 & 0.39 & 12 & 178 & 14 \\ 
   \hline
\hline
\end{longtable}


==> plots/plots/intervalploterror.tex <==
\begin{tikzpicture}
    \pgfplotsset{
        tmhplot/.style={color=red,opacity = .5,mark=none,line width=6pt,<->},
        omhplot/.style={color=blue,opacity = .5, mark=none,line width=6pt,<->},
        soldot/.style={color=red,only marks,mark=*},
        holdot/.style={color=red,fill=white,only marks,mark=*},
    }
        \begin{axis}[
                xmode = log,
                %width = .9\textwidth,
                %height = .25 \textheight,
                yticklabel style={rotate = 50, anchor = east},
                scaled y ticks=false,
                xmin=0,xmax=3,
                ymin=790,ymax=1010,
                legend pos = south east,
                ytick = {850,900,950,1000},
                %,1050,1100,1150
                yticklabels = {$800-850$,$850-900$,$900-950$,$950-1000$},
                %$1000-1050$,$1050-1100$,$1100-1150$
                ylabel = {Bins for Absolute Error $(\|x_k - x^*\|_2^2)$},
                ylabel style = {anchor = near ticklabel},
                xlabel = {Norm Squared of Gradient},
                title = {$90\%$ Intervals of Gradients Values at Different Error Ranges}
            ]
            %\addplot[omhplot,-,domain=2.24:2.24]{1050};
            
            %\addplot[tmhplot,-,domain=2.09:2.09]{1050};
            
            
            %\addplot[omhplot,-,domain=37.6:37.6]{1150};
            %\addplot[tmhplot,-,domain=32.6:32.6]{1150};
            
            \addplot[omhplot,-,domain=.00245:.0150]{850};
            \addlegendentry{Sketch Grad};
            \addplot[tmhplot,-,domain=.00348:.0132]{850};
            \addlegendentry{True Grad};
            
            \addplot[omhplot,-,domain=.0129:.0771]{900};
            \addplot[tmhplot,-,domain=.0164:.0752]{900};
            
            \addplot[omhplot,-,domain=.0838:.420]{950};
            \addplot[tmhplot,-,domain=.0974:.286]{950};
            
            \addplot[omhplot,-,domain=.446:1.03]{1000};
            \addplot[tmhplot,-,domain=.458:.817]{1000};
            
            %\addplot[omhplot,-,domain=973:1114]{.007};
            %\addplot[tmhplot,-,domain=1011:1120]{.007};
            
        \end{axis}

==> sections/experiments_theory-verification.tex <==
\section{Verification of Theory}\label{subsec:verify_th}
To verify our underlying theory that $\hat \rho_k^\lambda$ is consistent, our uncertainty sets cover at the appropriate rate, and the stopping conditions fail at the appropriate rates, it is necessary to design an experiment that takes the conditioning on $\siga$ into account. We design such an experiment using Johnson-Lindenstrauss sketches of an underlying linear system as described in \ref{ex:diff_priv}. In this setting, we have an underlying linear system, which we sketch. We repeatedly perform these sketches with sketching matrices that satisfy \cref{def:JL}, resulting in a stream of linear systems that have many fewer rows than the original. 

Under this setting the three sketching matrices included in \tref{table-eta} are each applied to 40 matrix systems from the \textit{MatrixDepot} library \cite{matrixdepot} resulting in 120 unique experimental observations of \cref{algo:Adaptive-window}. For each experimental observation, once the desired matrix type and sketching method has been chosen, the following two-stage experiment is performed with a constant moving average window width of $\lambda = 15$.
\begin{experiment}\label{exp:ther}
    Given $\lambda$, the sketching method, and linear system from \textit{MatrixDepot} we:

    \textbf{Stage 1:} 
        \begin{enumerate}
            \item Generate a matrix, $A \in \mathbb{R}^{256 \times 256}$, for the chosen linear system.
            \item Generate, $x^* \in \mathbb{R}^{256}$ with random entries from a Uniform(0,1).
            \item Generate the constant vector, $b = Ax^*$.
            \item Generate $\lbrace S_k \rbrace \subset \mathbb{R}^{25 \times 256}$ using the chosen sketching method. 
            \item Multiply $(A,b)$ from the left by $S_k$ to generate $(\tilde A_k, \tilde b_k) \in \mathbb{R}^{25 \times 256} \times \mathbb{R}^{25}$.
            \item Run \cref{algo:Adaptive-window} for 300 iterations using $(\tilde A_k, \tilde b_k)$'s and saving all the $x_k$'s.
        \end{enumerate}

    \textbf{Stage 2:}
    \begin{enumerate}
        \item Starting at each $x_k$, rerun \cref{algo:Adaptive-window} for $\lambda$ iterations, saving $\|\tilde r_k\|_2^2$ and $\|\tilde r_k\|_2^4$ at each iteration.  
        \item Use the $\|\tilde r_k\|_2^2$'s to compute $\hat \rho_k^\lambda$.
        \item Use the $\|\tilde r_k\|_2^4$'s to compute $\hat \iota_k^\lambda$. 
        \item Repeat steps 1-3, 100 independent times.
        \item For each $x_k$ average the 100 $\hat \rho_k^\lambda$'s to estimate $\rho_k^\lambda$.
    \end{enumerate}
\end{experiment}
\begin{table}[!hb]
    \caption{Conservative choices of the contraction parameter, $\eta$, by sketching method based on the experiment in \cref{exp:ther}.\protect\footnotemark}
    \label{table-eta}
    \centering
    \begin{tabular}{llll}
        \toprule
        \textbf{Sampling Method} & Achlioptas \cite{ACHLIOPTAS2003671} & FJLT \cite{Ailon2009TheFJ}  & Gaussian \cite{Dasgupta2003AnEP}\\
        \midrule
          $\eta$ & $26$ & $188$ & $26$\\
        \bottomrule
    \end{tabular} 
  \end{table}\footnotetext{By conservative, we mean that these are choices of $\eta$ that are the largest integer such that the coverage failure rate of the interval is as large as possible, but still less than the designed rate.} 
\subsection{Consistency of the Estimator}\label{subsec:conc_e}
\cref{cor:cons-of-rho} shows that the convergence of $\hat \rho_k^\lambda$ is dependent on the convergence of the iterates of \cref{algo:Adaptive-window}. Such dependency leads us to consider whether the relative errors between $\hat \rho_k^\lambda$ and $\rho_k^\lambda$ are bounded. By looking at the max, min, and median relative error for all the $\hat \rho_k^\lambda$s in the left plot of \fref{fig:estim}, we see that they all make minor oscillations around a constant, and thus we can conclude they are bounded. This boundedness implies that the absolute error decreases at a rate proportional to $\rho_k^\lambda$, an implication we verify using a Rohess matrix system with Gaussian sketching whose results displayed in right plot of \fref{fig:estim}. 
In this plot, the dotted line represents the value of $\rho_k^\lambda$ and the orange line represents the absolute error between the maximum absolute error of $\rho_k^\lambda$ and the 100 $\hat \rho_k^\lambda$s at each iteration. Taken together, we can conclude that $\hat \rho_k^\lambda$ is a consistent estimator for $\rho_k^\lambda$ and that it performs well in practice.




\begin{figure}[htb]
    \centering
    \Cinput{plots/conv_rho_plot.tex}
    \Cinput{plots/rhoViota.tex}
    \caption{The left plot shows relative error plot of the min (red), median (blue), and max (green) of the relative error between the $\rho_k^\lambda$ and $\hat \rho_k^\lambda$ across the 120 linear system and sketching method combinations.  The right plot shows the values of $\rho_k^\lambda$, dotted line, and the maximum absolute error at each iteration between all 100 $\hat \rho_k^\lambda$s and $\rho_k^\lambda$, the orange line.}\label{fig:estim}  
\end{figure}

\subsection{Validity of the Uncertainty Sets}\label{exp:uncer}
We next move to examining if the uncertainty sets cover $\rho_k^\lambda$ at the appropriate rate. To do this at each iteration of \cref{exp:ther} we compute the uncertainty sets with $\alpha = .05$ as described in \cref{algo:Adaptive-window} for each of the 100 $\hat \rho_k^\lambda$s. Then we examine how often these uncertainty sets fail to cover that iteration's $\rho_k^\lambda$. For all observations $\hat \rho_k^\lambda$, when $\eta = 1$ the coverage failure rate is $0.000773$ allowing us to conclude that the intervals are conservative, meaning they fail to cover $\rho_k^\lambda$ at a rate lower than what they are designed. We can mitigate this conservativeness, by setting $\eta$  according to \tref{table-eta}, resulting in failure rates of $0.052$ matching the designed failure rate for the uncertainty sets. 

Visually we represent some of these results by displaying the infimum of the upper bounds at each iteration, the supremum of lower bounds at each iteration, and the $\rho_k^\lambda$ at each iteration for the Wilkinson and Rohess linear systems solved with Gaussian sketching in \fref{fig:repsam}. Any time $\rho_k^\lambda$ exceeds these bounds the $\rho_k^\lambda$ point in the plot is marked in red, otherwise it is marked in green. From these figures we can see that with $\eta = 1$ the uncertainty sets are conservative since they cover $\rho_k^\lambda$ at all iterations. While when $\eta$ is set according to \tref{table-eta} for the  Wilkinson matrix we observe that $\rho_k^\lambda$  exceeds $0.0037$ of the $30,000$ uncertainty sets, while for the Rohess matrix $\rho_k^\lambda$ still fails to exceed any of the sets. This in total indicates that the uncertainty sets even with appropriately selected $\eta$ terms can be quite conservative, but nonetheless effective.

\begin{figure}
    \centering
    \Cinput{plots/rohess_rep.tex}
    \Cinput{plots/wilk_rep.tex}
    \caption{Coverage results for the uncertainty sets with $\alpha = 0.05$. The black line represent the infimum of the upper bounds. The plots on the left display the coverage when the uncertainty sets are calculated with $\eta = 1$, while those on the right are computed with $\eta$ set according to \tref{table-eta} based on some validation experiments. The green points display all the values of $\rho_k^\lambda$ that remain within the uncertainty set, while the red points are the values of $\rho_k^\lambda$ that fall outside the uncertainty set. The failure rates when $\eta = 1$  for the Rohess and  Wilkinson matrices with Gaussian sketching are $(0,0)$ respectively, while when the $\eta$ parameter is set according to \tref{table-eta} these values change to $(0,0.0037)$.} 
    \label{fig:repsam}
\end{figure}

\subsection{Validity of the Stopping Criterion}

Finally, we use the results of \cref{exp:ther} to verify if the stopping criterion appropriately controls the stopping errors. As a reminder,  the practical version of our stopping criterion is successful given user controlled parameters
$(\upsilon,\delta_I,\delta_{II}, \xi_I, \xi_{II})=(100,0.9, 1.1, 0.01, 0.01)$ if it is the case that both 
\begin{eqnarray}
    &\mathbb{P}\left[ \hat \rho_{k+1}^\lambda > \upsilon, \rho_k^\lambda \leq \delta_I\upsilon \bigg{\vert} \mathcal{F}_{k-\lambda+1} \right] < \xi_I \label{eq:early} \text{ and} \\ 
    &\mathbb{P}\left[ \hat \rho_{k+1}^\lambda \leq  \upsilon, \rho^\lambda_k > \delta_{II} \upsilon \bigg{\vert} \mathcal{F}_{k-\lambda+1} \right] < \xi_{II} \label{eq:late},
\end{eqnarray}
are satisfied when the while loop condition in Line \ref{stopping-condition} of \cref{algo:Adaptive-window} is violated, i.e. the stopping criterion is satisfied. This means that to verify the theory we just need to compute the rates of \ref{eq:early} and \ref{eq:late} when the stopping condition is satisfied and verify that it is less than $\xi_I$ and $\xi_{II}$. When we compute these rates with $\eta = 1$ we can see that in \fref{fig:stoppingplot} that no stopping error of either type occurs. The lack of failures continues to be true even when $\eta$ is set  according to \tref{table-eta}; thus, we can conclude that our stopping criterion is effective and well controls the stopping errors. 

\begin{figure}
    \centering
    \Cinput{plots/stopping_plot.tex} 
    \caption{Graph depicting the stopping decision results by error type. The late category describes an error of the form \ref{eq:early}, while early describes an error of the form  \ref{eq:late}. These results are displayed with $\eta = 1$; however, they remain unchanged even if $\eta$ is set according to \tref{table-eta}.}
    \label{fig:stoppingplot}
\end{figure}

